CANIFE: Crafting Canaries for Empirical Privacy Measurement in Federated Learning

Federated Learning (FL) is a setting for training machine learning models in distributed environments where the clients do not share their raw data but instead send model updates to a server. However, model updates can be subject to attacks and leak private information. Differential Privacy (DP) is a leading mitigation strategy which involves adding noise to clipped model updates, trading off performance for strong theoretical privacy guarantees. Previous work has shown that the threat model of DP is conservative and that the obtained guarantees may be vacuous or may overestimate information leakage in practice. In this paper, we aim to achieve a tighter measurement of the model exposure by considering a realistic threat model. We propose a novel method, CANIFE, that uses canaries - carefully crafted samples by a strong adversary to evaluate the empirical privacy of a training round. We apply this attack to vision models trained on CIFAR-10 and CelebA and to language models trained on Sent140 and Shakespeare. In particular, in realistic FL scenarios, we demonstrate that the empirical per-round epsilon obtained with CANIFE is 4-5x lower than the theoretical bound.

==> comments.tex <==
Writing Plan:
\begin{itemize}
    \item Meeting (12/09/22)
    \begin{enumerate}
        \item \st{Background: Cut down 2.2}
        \item \st{Background: Cut down 2.3}
        \item \st{Cleanup "measuring privacy", define $s_r$ or not?}
        \item \st{Empirical epsilon notation: Will we use both per-step and global? Just global?}
        \item \st{ $\alpha^2||\canarygrad||^2 = 1$ assumption: Maybe be less precise about this}
        \item \st{Start experiment write up: CIFAR10 $\rightarrow$ Measuring Privacy $\rightarrow$ Ablations}
        \item Threat model: Table/Figure to summarise?
        \item Methodology: user-level/sample-level discussion - need to be clear about designing and modifying a sample to give user-level guarantees
        \item Add reference in methodology that normalising canary grad during optimisation helps and refer to plot in Appendix
    \end{enumerate}
\end{itemize}


Experiments Plan:
\begin{itemize}
    \item CIFAR10 Toy Experiment
    \item Monitoring Privacy 
    \item Ablation Study:
    \begin{itemize}
        \item Main paper
        \begin{itemize}
            \item Image (text) vs Random initialisation
            \item Design pool size
            \item Number of clients + local updates
            \item Effect of canary iterations (+ design time)  
            \item Insert epoch/model accuracy correlated with attack accuracy
        \end{itemize}
        \item Appendix
        \begin{itemize}
            \item Loss 1 vs Loss 2
            \item Normalisation of gradient
            \item Design on ImageNet (cats / dogs classes vs CIFAR10)
            \item (?) Effect of canary norm term(s)
            \item (?) Vary canary norm constant?
            \item (?) Sample gradients vs model updates
        \end{itemize}
    \end{itemize}
\end{itemize}

Appendix:
\begin{itemize}
    \item LRT section
    \item Model architectures + training details
    \item Further ablations
    \begin{itemize}
        \item 'for designing the canary such as batching mock client updates, slightly modifying the loss and different insertion strategies.'
    \end{itemize}
    \item 
\end{itemize}
